Speed/accuracy trade-offs for modern convolutional object detectors

The goal of this paper is to serve as a guide for selecting a detection architecture that achieves the right speed/memory/accuracy balance for a given application and platform. To this end, we investigate various ways to trade accuracy for speed and memory usage in modern convolutional object detection systems. A number of successful systems have been proposed in recent years, but apples-to-apples comparisons are difficult due to different base feature extractors (e.g., VGG, Residual Networks), different default image resolutions, as well as different hardware and software platforms. We present a unified implementation of the Faster R-CNN [Ren et al., 2015], R-FCN [Dai et al., 2016] and SSD [Liu et al., 2015] systems, which we view as "meta-architectures" and trace out the speed/accuracy trade-off curve created by using alternative feature extractors and varying other critical parameters such as image size within each of these meta-architectures. On one extreme end of this spectrum where speed and memory are critical, we present a detector that achieves real time speeds and can be deployed on a mobile device. On the opposite end in which accuracy is critical, we present a detector that achieves state-of-the-art performance measured on the COCO detection task.

==> commands.tex <==
\usepackage[T1]{fontenc}
\usepackage[latin1]{inputenc}
\usepackage{amssymb}
\usepackage{amsmath}
%\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{graphicx}
%\usepackage[boxed,noend]{algorithm2e}

%\usepackage[algo2e,noend,linesnumbered,boxed]{algorithm2e}
\usepackage[algo2e,noend,boxed]{algorithm2e}
\usepackage{algorithmic}
\usepackage{algorithm}

\usepackage{xspace}
\usepackage{dsfont}
%\usepackage{fullpage}
\usepackage{graphicx}  
\usepackage{verbatim}
\usepackage{appendix}
\usepackage{multirow}
\usepackage{color}
\usepackage{framed}
\usepackage{wrapfig}
\newtheorem{thm}{Theorem}%[section]
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{prob}[thm]{Problem}
\newtheorem{example}[thm]{Example}
%\theoremstyle{definition}
%\newtheorem{defn}[thm]{Definition}
%\theoremstyle{remark}
%\newtheorem{rem}[thm]{Remark}

%\newcommand{\shadecolor}{white}
\definecolor{shadecolor}{rgb}{.6,.6,.6}
\newenvironment{highlight}[1][gray]%
 {\vspace*{0.5\baselineskip}
\begin{center}\begin{minipage}{0.85\textwidth}\begin{shaded}}%
 {\end{shaded}\end{minipage}\end{center} \vspace*{0.5\baselineskip}}

% enable subfigures
\usepackage[tight,scriptsize]{subfigure}
%\usepackage{subfloat}
\newcommand{\denselist}{
\itemsep -2pt\topsep-8pt\partopsep-8pt
}
\newcommand{\loud}[1]{\textcolor{green}{!!!! #1 !!!!}}

\newcommand{\Jon}[1]{{\color{red}{\bf\sf [Jon: #1]}}}
\newcommand{\Kevin}[1]{{\color{blue}{\bf\sf [Kevin: #1]}}}
\newcommand{\kevin}[1]{{\color{blue}{\bf\sf [Kevin: #1]}}}
\newcommand{\eat}[1]{}

\vfuzz2pt % Don't report over-full v-boxes if over-edge is small
\hfuzz2pt % Don't report over-full h-boxes if over-edge is smallq
\numberwithin{equation}{section}
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\blankbox}[2]{%
  \parbox{\columnwidth}{\centering
    \setlength{\fboxsep}{0pt}%
    \fbox{\raisebox{0pt}[#2]{\hspace{#1}}}%
  }%
}
\newcommand{\blockcomment}[1]{ }

\newcommand{\tr}{\mbox{Tr }}
\newcommand{\bfi}{\bfseries\itshape}
\def\reals{\mathbb{R}}
\def\rationals{\mathbb{Q}}
\def\borel{\mathbb{B}}
\newcommand{\complex}{\mathbb{C}}
\newcommand{\eqbase}{1/2}
\newcommand{\eqalt}{\sqrt{3}/2}
\newcommand{\im}{\mbox{im }}
\def\naturals{\mathbb{N}}
\def\expectation{\mathbb{E}}
\def\normal{\mathcal{N}}
\def\Tr{\mbox{Tr}}
\def\triv{{\bf 1}}

\newcommand{\drho}[1]{d_{\rho_{#1}}}
\newcommand{\twovec}[2]{\left[
\begin{array}{c}
#1 \\
#2 \\
\end{array}\right]
}
\newcommand{\twomat}[4]{\left[
\begin{array}{cc}
#1 & #2 \\
#3 & #4 \\
\end{array}\right]
}
\newcommand{\threemat}[9]{\left[
\begin{array}{ccc}
#1 & #2 & #3 \\
#4 & #5 & #6 \\
#7 & #8 & #9 \\
\end{array}
\right]
}
\newcommand{\threematbl}[4]{\left[
\begin{array}{cccc}
1 & \vline & 0 & 0 \\
\hline
0 & \vline & #1 & #2 \\
0 & \vline & #3 & #4 \\
\end{array}
\right]
}
\def\triv{{\bf 1}}
\def\post{\widehat{L^{(t)}P^{(t)}}}
\def\postbra{\left[\post\right]}
\newcommand{\Conditioning}{{\sc KroneckerConditioning} \xspace}
\newcommand{\PredictionRollup}{{\sc PredictionRollup} \xspace}
\newcommand{\ComputeCG}{{\sc ClebschGordanCoeffs} \xspace}
\newcommand{\ind}[1]{\mathds{1}\left\{#1\right\}}
\newcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\invFourier}[3]{
\hat{#1}_{\rho_{#3}}^T \cdot #2_{#3}(\sigma)
}

\newbox\subfigbox
\makeatletter
\newenvironment{subfloat}
{\def\caption##1{\gdef\subcapsave{\relax##1}}%
\let\subcapsave\@empty\setbox\subfigbox\hbox
\bgroup}{\egroup\subfigure[\subcapsave]{\box\subfigbox}}
\makeatother

\newcommand\T{\rule{0pt}{3.7ex}} %top strut
\newcommand\B{\rule[-3.1ex]{0pt}{0pt}} %bottom strut
\newcommand\TT{\rule{0pt}{2.7ex}} %top strut
\newcommand\BB{\rule[-1.8ex]{0pt}{0pt}} %bottom strut


